Imaging-anchored multiomics in cardiovascular disease: integrating cardiac imaging, bulk, single-cell, and spatial transcriptomics

Cardiovascular disease arises from interactions between inherited risk, molecular programmes, and tissue-scale remodelling that are observed clinically through imaging. Cardiac MRI (CMR), computed tomography (CT), and echocardiography are integral to routine cardiovascular care, while bulk RNA sequencing, single-cell RNA sequencing, and spatial transcriptomics are providing increasingly detailed molecular characterization of cardiac tissue. Yet, these imaging and molecular data are still analysed in largely separate pipelines. This review examines joint representations that link cardiac imaging phenotypes to transcriptomic and spatially resolved molecular states. An imaging-anchored perspective is adopted in which echocardiography, CMR, and CT define a spatial phenotype of the heart, and bulk, single-cell and spatial transcriptomics provide cell-type- and location-specific molecular context. We define the representation requirements of each modality, compare multimodal fusion strategies, and synthesize integrative pipelines for radiogenomics, spatial alignment, and image-based gene-expression prediction, together with their validation requirements, limitations, and failure modes. Spatial multiomic maps of human myocardium and atherosclerotic plaque, together with single-cell, spatial, and multimodal medical foundation models, are advancing imaging-anchored multiomics; however, cost, scalability, and tissue availability remain substantial barriers to large-scale cardiovascular translation.

==> BIB_Review_Bioinformatics_MinhLe_UPDATED/figures/figure-1.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figure_1.jpg}
\caption{The resolution scale illustrates the gap between in vivo cardiac imaging at centimetre-to-millimetre resolution and molecular spatial profiling, from Visium 55 \textmu{}m spots and Visium HD/Stereo-seq 2-8 \textmu{}m bins to single-cell platforms such as Xenium and MERSCOPE. Cardiac imaging modalities, including echocardiography, cardiac magnetic resonance imaging (CMR), and cardiac CT/CTA, define spatial phenotypes of the heart using measures such as ejection fraction, global longitudinal strain, wall motion, late gadolinium enhancement, T1 mapping, cine imaging, plaque features, fat attenuation index, and coronary artery calcium. These phenotypes can be indexed at the voxel, American Heart Association segment, or joint latent-space level and linked to molecular omics layers, including spatial transcriptomics, bulk or single-nucleus RNA sequencing, and proteomics/spatial omics. The resulting joint representations support downstream tasks including clinical prediction, virtual transcriptomics, spatial alignment, radiogenomics, and multimodal fusion. Foundation models spanning single-cell/spatial omics, vision--omics, imaging, and medical multimodal data provide computational support across the framework. Applications include disease subtyping, mechanism discovery, biomarker prioritisation, and risk prediction. Abbreviations: AHA, American Heart Association; CMR, cardiac magnetic resonance imaging; CT, computed tomography; CTA, computed tomography angiography; EF, ejection fraction; GLS, global longitudinal strain; LGE, late gadolinium enhancement; FAI, fat attenuation index; CAC, coronary artery calcium; scVI, single-cell variational inference; DCA, deep count autoencoder; DCCA, deep canonical correlation analysis; MOFA+, multi-omics factor analysis; VLM, vision--language model.}
\label{fig:imaging_anchored_framework}
\end{figure*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/figures/figure-2.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figure_2.jpg}
\caption{Multimodal fusion architectures for radiomics--omics integration. Panel (A): early fusion concatenates radiomics and omics feature vectors followed by a single predictive model. Panel (B): intermediate fusion uses modality-specific encoders and a shared latent space, often with reconstruction heads; the shared latent captures biology concordant across modalities while private components retain modality-specific information. Panel (C): late fusion combines predictions from separate radiomics and omics models via an ensemble or calibration layer; it is robust to missing modalities but cannot capture cross-modal feature interactions. Panel (D): graph-based and contrastive approaches construct cross-modal latent spaces using biological or spatial graphs and contrastive objectives.}
\label{fig:multimodal_fusion}
\end{figure*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/figures/figure-3.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figure_3.jpg}
\caption{Archetypal pipelines for imaging--omics integration. Radiogenomics workflows link imaging-derived features to bulk or single-cell molecular profiles via feature extraction, joint latent modelling, and association or causal inference; spatial molecular alignment pipelines register in vivo imaging, ex vivo imaging, histology and spatial transcriptomics into a common coordinate system; virtual transcriptomics approaches use deep models to predict molecular modules or spatial expression maps directly from imaging inputs.}
\label{fig:integration_pipelines}
\end{figure*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/figures/figure-4.tex <==
\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figure_4.jpg}
\caption{Translational roadmap from imaging-anchored multiomics to digital twins. Top lane: model stack comprising modality-specific encoders, multimodal fusion models and transformer or foundation model architectures. Middle lane: an agentic layer in which large language models orchestrate tool calls to encoders, fusion models and knowledge bases to generate structured reports and explanations. Bottom lane: translational path from data curation and model development through external validation and deployment to decision support and digital twin--enabled in silico trials.}
\label{fig:translational_roadmap}
\end{figure*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/frontmatter.tex <==
\journaltitle{Briefings in Bioinformatics}
\DOI{https://doi.org/10.1093/bib/bbag365}
\copyrightyear{2026}
\pubyear{2026}
\volume{27}
\vol{27}
\issue{4}
\appnotes{Review}
\firstpage{1}
\title{Imaging-anchored multiomics in cardiovascular disease: integrating cardiac imaging, bulk, single-cell, and spatial transcriptomics}

\author[1]{Minh H. N. Le}
\author[2]{Thanh-Huy Nguyen}
\author[3]{Tao Li}
\author[4]{Bao Quang Gia Le}
\author[5]{Han H. Huynh}
\author[4]{Monika Raj}
\author[3]{Carl Yang}
\author[2]{Min Xu}
\author[6,*]{Tuan Vinh}
\author[7,8,9,*]{Nguyen Quoc Khanh Le}

\address[1]{Section of Cardiovascular Medicine, Department of Internal Medicine, Yale School of Medicine, 333 Cedar Street, New Haven, CT 06510, United States}
\address[2]{Computational Biology Department, School of Computer Science, Carnegie Mellon University, 5000 Forbes Avenue, Pittsburgh, PA 15213, United States.}
\address[3]{Department of Computer Science, Emory University, 201 Dowman Drive, Atlanta, GA 30322, United States}
\address[4]{Department of Chemistry, Emory University, 1515 Dickey Drive, Atlanta, GA 30322, United States}
\address[5]{Irell and Manella Graduate School of Biological Science, City of Hope, CA, United States}
\address[6]{Medical Sciences Division, University of Oxford, John Radcliffe Hospital, Headington, Oxford OX3 9DU, Oxfordshire, United Kingdom}
\address[7]{AIBioMed Research Group, Taipei Medical University, 250 Wu-Hsing Street, Xinyi District, Taipei 11031, Taiwan}
\address[8]{In-Service Master Program in Artificial Intelligence in Medicine, College of Medicine, Taipei Medical University, 250 Wu-Hsing Street, Xinyi District, Taipei 11031, Taiwan}
\address[9]{Translational Imaging Research Center, Taipei Medical University Hospital, 252 Wu-Hsing Street, Xinyi District, Taipei 11031, Taiwan}
\corresp[*]{Corresponding authors. Tuan Vinh, Medical Sciences Division, University of Oxford, John Radcliffe Hospital, Headington, Oxford OX3 9DU, Oxfordshire, United Kingdom. E-mail: \href{mailto:tuan.vinh@hertford.ox.ac.uk}{tuan.vinh@hertford.ox.ac.uk}; Nguyen Quoc Khanh Le, In-Service Master Program in Artificial Intelligence in Medicine, College of Medicine, Taipei Medical University, Taipei, Taiwan. E-mail: \href{mailto:khanhlee@tmu.edu.tw}{khanhlee@tmu.edu.tw}.}

\abstract{Cardiovascular disease arises from interactions between inherited risk, molecular programmes, and tissue-scale remodelling that are observed clinically through imaging. Cardiac MRI (CMR), computed tomography (CT), and echocardiography are integral to routine cardiovascular care, while bulk RNA sequencing, single-cell RNA sequencing, and spatial transcriptomics are providing increasingly detailed molecular characterization of cardiac tissue. Yet, these imaging and molecular data are still analysed in largely separate pipelines. This review examines joint representations that link cardiac imaging phenotypes to transcriptomic and spatially resolved molecular states. An imaging-anchored perspective is adopted in which echocardiography, CMR, and CT define a spatial phenotype of the heart, and bulk, single-cell and spatial transcriptomics provide cell-type- and location-specific molecular context. We define the representation requirements of each modality, compare multimodal fusion strategies, and synthesize integrative pipelines for radiogenomics, spatial alignment, and image-based gene-expression prediction, together with their validation requirements, limitations, and failure modes. Spatial multiomic maps of human myocardium and atherosclerotic plaque, together with single-cell, spatial, and multimodal medical foundation models, are advancing imaging-anchored multiomics; however, cost, scalability, and tissue availability remain substantial barriers to large-scale cardiovascular translation.}
\maketitle


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/key-points.tex <==
\par\vspace{10bp}
\noindent\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\fontsize{7.5bp}{11bp}\selectfont
\textbf{Key Points}
\begin{itemize}
\item Imaging-anchored multiomics learns joint representations linking cardiac imaging phenotypes to bulk, sc/snRNA-seq, and spatial transcriptomics.
\item Cardiac imaging provides a spatial phenotype that supports voxel/region alignment with molecular states and cell-type programmes.
\item Fusion methods can accommodate missing modalities and batch effects but remain constrained by small paired cohorts.
\item Applications include radiogenomics, virtual transcriptomics, disease subtyping, mechanism discovery, and biomarker prioritization for cardiovascular disease.
\end{itemize}
\end{minipage}}
\par\vspace{8bp}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/published-references.tex <==
% Published reference wording, numbering and typography; original citation keys retained.
\begin{thebibliography}{128}

\bibitem{world_heart_statistics}
Global Burden of Cardiovascular Diseases and Risks 2023 Collaborators. Global, regional, and national burden of cardiovascular diseases and risk factors in 204 countries and territories, 1990--2023. \textit{J Am Coll Cardiol} 2025;\textbf{86}:2167--2243.

\bibitem{litvivnukova2020cells}
Litviňuková M, Talavera-López C, Maatz H \textit{et al}. Cells of the adult human heart. \textit{Nature} 2020;\textbf{588}:466--72.

\bibitem{tucker2020transcriptional}
Tucker NR, Chaffin M, Fleming SJ \textit{et al}. Transcriptional and cellular diversity of the human heart. \textit{Circulation} 2020;\textbf{142}:466--82.

\bibitem{leiner2019machine}
Leiner T, Rueckert D, Suinesiaputra A \textit{et al}. Machine learning in cardiovascular magnetic resonance: basic concepts and applications. \textit{J Cardiovasc Magn Reson} 2019;\textbf{21}:61.

\bibitem{ouyang2020_echonet_dynamic}
Ouyang D, He B, Ghorbani A \textit{et al}. Video-based AI for beat-to-beat assessment of cardiac function. \textit{Nature} 2020;\textbf{580}:252--6.

\bibitem{zhou2025_multimodal_cad_review}
Zhou Z, Wang J. A narrative review of multimodal data fusion strategies for precision risk prediction in coronary artery disease: advances, challenges, and future informatics directions. \textit{Rambam} \textit{Maimonides Med J} 2025;\textbf{16}:e0023.

\bibitem{spatial_heart_review_2025}
Farah EN, Diaz JT, Bloomekatz J \textit{et al}. Charting the cardiac landscape: advances in spatial transcriptomics for heart biology. \textit{Semin} \textit{Cell Dev Biol} 2025;\textbf{175}:103648.

\bibitem{moor2023_foundation_models}
Moor M, Banerjee O, Abad ZSH \textit{et al}. Foundation models for generalist medical artificial intelligence. \textit{Nature} 2023;\textbf{616}:259--65.

\bibitem{tu2024_generalist_biomed_ai}
Tu T, Azizi S, Driess D \textit{et al.} Towards generalist biomedical AI. \textit{NEJM} \textit{AI} 2024;\textbf{1}:AIoa2300138.

\bibitem{lim2025practical}
Lim HJ, Wang Y, Buzdin A \textit{et al}. A practical guide for choosing an optimal spatial transcriptomics technology from seven major commercially available options. \textit{BMC Genomics} 2025;\textbf{26}:47.

\bibitem{pentimalli2025challenges}
Pentimalli TM, Karaiskos N, Rajewsky N. Challenges and opportunities in the clinical translation of high-resolution spatial transcriptomics. \textit{Annu Rev Pathol} 2025;\textbf{20}:405--32.

\bibitem{kuppe2022_spatial_mi}
Kuppe C, Ramirez Flores RO, Li Z \textit{et al}. Spatial multi-omic map of human myocardial infarction. \textit{Nature} 2022;\textbf{608}:766--77.

\bibitem{calcagno2022_infarct_spatial}
Calcagno DM, Taghdiri N, Ninh VK \textit{et al}. Single-cell and spatial transcriptomics of the infarcted heart define the dynamic onset of the border zone in response to mechanical destabilization. \textit{Nat} \textit{Cardiovasc Res} 2022;\textbf{1}:1039--55.

\bibitem{unterberg2017targeted}
Unterberg-Buchwald C, Ritter CO, Reupke V \textit{et al}. Targeted endomyocardial biopsy guided by real-time cardiovascular magnetic resonance. \textit{J Cardiovasc Magn Reson} 2017;\textbf{19}:45.

\bibitem{lurz2012diagnostic}
Lurz P, Eitel I, Adam J \textit{et al}. Diagnostic performance of CMR imaging compared with EMB in patients with suspected myocarditis. \textit{JACC} \textit{Cardiovasc Imaging} 2012;\textbf{5}:513--24.

\bibitem{duffy2022high}
Duffy G, Cheng PP, Yuan N \textit{et al}. High-throughput precision phenotyping of left ventricular hypertrophy with cardiovascular deep learning. \textit{JAMA Cardiol} 2022;\textbf{7}:386--95.

\bibitem{petersen2013imaging}
Petersen SE, Matthews PM, Bamberg F \textit{et al}. Imaging in population science: cardiovascular magnetic resonance in 100,000 participants of UK Biobank-rationale, challenges and approaches. \textit{J} \textit{Cardiovasc Magn Reson} 2013;\textbf{15}:46.

\bibitem{ferencik2018use}
Ferencik M, Mayrhofer T, Bittner DO \textit{et al}. Use of high-risk coronary atherosclerotic plaque detection for risk stratification of patients with stable chest pain: a secondary analysis of the PROMISE randomized clinical trial. \textit{JAMA Cardiol} 2018;\textbf{3}:144--52.

\bibitem{radiomics_cmr_2020}
Cetin I, Raisi-Estabragh Z, Petersen SE \textit{et al}. Radiomics signatures of cardiovascular risk factors in cardiac MRI: results from the UK biobank. \textit{Front Cardiovasc Med} 2020;\textbf{7}:591368.

\bibitem{kuruvilla2014_lge_meta}
Kuruvilla S, Adenaw N, Katwal A \textit{et al}. Late gadolinium enhancement on cardiac magnetic resonance predicts adverse cardiovascular outcomes in nonischemic cardiomyopathy: a systematic review and meta-analysis. \textit{Circ Cardiovasc Imaging} 2014; \textbf{7}:250--8.

\bibitem{kalam2014_gls_meta}
Kalam K, Otahal P, Marwick TH. \textit{Prognostic implications of global LV dysfunction: a systematic review and meta-analysis of global longitudinal strain and ejection fraction. Heart} 2014;\textbf{100}:1673--80.

\bibitem{williams2020_scotheart_lap}
Williams MC, Kwiecinski J, Doris M \textit{et al}. Low-attenuation noncalcified plaque on coronary computed tomography angiography predicts myocardial infarction: results from the multicenter SCOT-HEART trial. \textit{Circulation} 2020;\textbf{141}:1452--62.

\bibitem{otsuka2013_napkin_ring}
Otsuka K, Fukuda S, Tanaka A \textit{et al}. Napkin-ring sign on coronary CT angiography for the prediction of acute coronary syndrome. \textit{JACC Cardiovasc Imaging} 2013;\textbf{6}:448--57.

\bibitem{oikonomou2018_pv_fai_risk}
Oikonomou EK, Marwan M, Desai MY \textit{et al}. Non-invasive detection of coronary inflammation using computed tomography and prediction of residual cardiovascular risk (the CRISP CT study): a post-hoc analysis of prospective outcome data. \textit{Lancet} 2018;\textbf{392}: 929--39.

\bibitem{koenig2022_cardiomyopathy_rnaseq}
Koenig AL, Shchukina I, Amrute J \textit{et al}. Single-cell transcriptomics reveals cell-type-specific diversification in human heart failure. \textit{Nat Cardiovasc Res} 2022;\textbf{1}:263--80.

\bibitem{ganz2016_protein_risk_jama}
Ganz P, Heidecker B, Hveem K \textit{et al}. Development and validation of a protein-based risk score for cardiovascular outcomes among patients with stable coronary heart disease. \textit{JAMA} 2016;\textbf{315}:2532--41.

\bibitem{wang2020_hf_scseq}
Wang L, Peng Y, Zhou B \textit{et al}. Single-cell reconstruction of the adult human heart during heart failure and recovery reveals the cellular landscape underlying cardiac function. \textit{Nat Cell Biol} 2020;\textbf{22}:108--19.

\bibitem{lee2025_spatial_hf}
Lee SE, Joo JH, Hwang HS \textit{et al}. Spatial transcriptional landscape of human heart failure. \textit{Eur Heart J} 2025;\textbf{46}:3098--114.

\bibitem{campos2025_spatial_plaque}
Campos J, McMurray JL, Certo M \textit{et al}. Spatial transcriptomics elucidates localized immune responses in atherosclerotic coronary artery. \textit{EMBO Mol Med} 2025;\textbf{17}:2827--46.

\bibitem{kleshchevnikov2022cell2location}
Kleshchevnikov V, Shmatko A, Dann E \textit{et al}. Cell2location maps fine-grained cell types in spatial transcriptomics. \textit{Nat Biotechnol} 2022;\textbf{40}:661--71.

\bibitem{bild2002_mesa}
Bild DE, Bluemke DA, Burke GL \textit{et al}. Multi-ethnic study of atherosclerosis: objectives and design. \textit{Am J Epidemiol} 2002;\textbf{156}:871--81.

\bibitem{kramer2015_hcmr}
Kramer CM, Appelbaum E, Desai MY \textit{et al}. Hypertrophic cardiomyopathy registry: the rationale and design of an international, observational study of hypertrophic cardiomyopathy. \textit{Am Heart J} 2015;\textbf{170}:223--30.

\bibitem{gow2023_mimic_iv_ecg}
Gow B, Pollard T, Nathanson LA \textit{et al.} MIMIC-IV-ECG: Diagnostic Electrocardiogram Matched Subset (version 1.0). \textit{PhysioNet} 2023. \url{https://doi.org/10.1111/10.13026/4nqg-sb35}.

\bibitem{fonseca2011_cardiac_atlas}
Fonseca CG, Backhaus U, Bluemke DA \textit{et al}. The cardiac atlas project---an imaging database for cardiovascular phenotypes. \textit{Bioinformatics} 2011;\textbf{27}:2288--95.

\bibitem{sun2023spatial}
Sun J, Singh P, Shami A \textit{et al}. Spatial transcriptional mapping reveals site-specific pathways underlying human atherosclerotic plaque rupture. \textit{J Am Coll Cardiol} 2023;\textbf{81}:2213--27.

\bibitem{gastanadui2024_coronary_spatial_plaque}
Gastanadui MG, Margaroli C, Litovsky S \textit{et al}. Spatial transcriptomic approach to understanding coronary atherosclerotic plaque stability. \textit{Arterioscler Thromb Vasc Biol} 2024;\textbf{44}:e264--76.

\bibitem{bai2018automated}
Bai W, Sinclair M, Tarroni G \textit{et al}. Automated cardiovascular magnetic resonance image analysis with fully convolutional networks. \textit{J Cardiovasc Magn Reson} 2018;\textbf{20}:65.

\bibitem{bai2020population}
Bai W, Suzuki H, Huang J \textit{et al}. A population-based phenome-wide association study of cardiac and aortic structure and function. \textit{Nat} \textit{Med} 2020;\textbf{26}:1654--62.

\bibitem{oikonomou2019novel}
Oikonomou EK, Williams MC, Kotanidis CP \textit{et al}. A novel machine learning-derived radiotranscriptomic signature of perivascular fat improves cardiac risk prediction using coronary CT angiography. \textit{Eur Heart J} 2019;\textbf{40}:3529--43.

\bibitem{dosovitskiy2021_vit}
Dosovitskiy A, Beyer L, Kolesnikov A \textit{et al.} An image is worth 16 $\times$ 16 words: transformers for image recognition at scale. In: \textit{International Conference on Learning Representations}. Virtual conference: OpenReview.net; 2021.

\bibitem{he2022_mae}
He K, Chen X, Xie S \textit{et al.} Masked autoencoders are scalable vision learners. In: Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition. New Orleans (LA), USA: IEEE; 2022. p. 15979--88.

\bibitem{jacob2025towards}
Jacob AJ, Borgohain I, Chitiboi T \textit{et al}. Towards a cardiovascular magnetic resonance foundation model for multi-task cardiac image analysis. \textit{J Cardiovasc Magn Reson} 2025;\textbf{27}:101967.

\bibitem{christensen2024vision}
Christensen M, Vukadinovic M, Yuan N \textit{et al}. Vision--language foundation model for echocardiogram interpretation. \textit{Nat Med} 2024;\textbf{30}:1481--8.

\bibitem{chen2025visual}
Chen W, Zhang P, Tran TN \textit{et al}. A visual--omics foundation model to bridge histopathology with spatial transcriptomics. \textit{Nat Methods} 2025;\textbf{22}:1568--82.

\bibitem{cisternino2024self}
Cisternino F, Ometto S, Chatterjee S \textit{et al}. Self-supervised learning for characterising histomorphological diversity and spatial RNA expression prediction across 23 human tissue types. \textit{Nat Commun} 2024;\textbf{15}:5906.

\bibitem{langfelder2008wgcna}
Langfelder P, Horvath S. WGCNA: an R package for weighted correlation network analysis. \textit{BMC Bioinformatics} 2008;\textbf{9}:559.

\bibitem{hao2024dictionary}
Hao Y, Stuart T, Kowalski MH \textit{et al}. Dictionary learning for integrative, multimodal and scalable single-cell analysis. \textit{Nat Biotechnol} 2024;\textbf{42}:293--304.

\bibitem{wolf2018scanpy}
Wolf FA, Angerer P, Theis FJ. SCANPY: Large-scale single-cell gene expression data analysis. \textit{Genome Biol} 2018;\textbf{19}:15.

\bibitem{eraslan2019single}
Eraslan G, Simon LM, Mircea M \textit{et al}. Single-cell RNA-seq denoising using a deep count autoencoder. \textit{Nat Commun} 2019;\textbf{10}:390.

\bibitem{lopez2018_scvi}
Lopez R, Regier J, Cole MB \textit{et al}. Deep generative modeling for single-cell transcriptomics. \textit{Nat Methods} 2018;\textbf{15}:1053--8.

\bibitem{gayoso2022_scvi_tools}
Gayoso A, Lopez R, Xing G \textit{et al}. A Python library for probabilistic analysis of single-cell omics data. \textit{Nat Biotechnol} 2022;\textbf{40}:163--6.

\bibitem{argelaguet2018_mofa}
Argelaguet R, Velten B, Arnol D \textit{et al}. Multi-omics factor analysis-a framework for unsupervised integration of multi-omics data sets. \textit{Mol Syst Biol} 2018;\textbf{14}:e8124.

\bibitem{singlecell_foundation_2024}
Hao M, Gong J, Zeng X \textit{et al}. Large-scale foundation model on single-cell transcriptomics. \textit{Nat Methods} 2024;\textbf{21}:1481--91.

\bibitem{nicheformer_2025}
Tejada-Lapuerta A, Schaar AC, Gutgesell R \textit{et al.} Nicheformer: a foundation model for single-cell and spatial omics. \textit{Nat Methods} 2025;\textbf{22}:2525--38.

\bibitem{hu2021_spagcn}
Hu J, Li X, Coleman K \textit{et al}. SpaGCN: integrating gene expression, spatial location and histology to identify spatial domains and spatially variable genes by graph convolutional network. \textit{Nat Methods} 2021;\textbf{18}:1342--51.

\bibitem{zhao2021spatial}
Zhao E, Stone MR, Ren X \textit{et al}. Spatial transcriptomics at subspot resolution with BayesSpace. \textit{Nat Biotechnol} 2021;\textbf{39}:1375--84.

\bibitem{dong2022deciphering}
Dong K, Zhang S. Deciphering spatial domains from spatially resolved transcriptomics with an adaptive graph attention auto-encoder. \textit{Nat Commun} 2022;\textbf{13}:1739.

\bibitem{long2023spatially}
Long Y, Ang KS, Li M \textit{et al}. Spatially informed clustering, integration, and deconvolution of spatial transcriptomics with GraphST. \textit{Nat Commun} 2023;\textbf{14}:1155.

\bibitem{zhou2025_stmsgal}
Zhou L, Peng X, Chen M \textit{et al}. Unveiling patterns in spatial transcriptomics data: a novel approach utilizing graph attention autoencoder and multiscale deep subspace clustering network. \textit{GigaScience} 2025;\textbf{14}:giae103.

\bibitem{min2024multimodal}
Min W, Shi Z, Zhang J \textit{et al}. Multimodal contrastive learning for spatial gene expression prediction using histology images. \textit{Brief} \textit{Bioinform} 2024;\textbf{25}:bbae551.

\bibitem{wang2025benchmarking}
Wang C, Chan AS, Fu X \textit{et al}. Benchmarking the translational potential of spatial gene expression prediction from histology. \textit{Nat} \textit{Commun} 2025;\textbf{16}:1544.

\bibitem{heist_2025}
Madhu H, Rocha JF, Huang T \textit{et al.} HEIST: a graph foundation model for spatial transcriptomics and proteomics data. In: \textit{The} \textit{Fourteenth International Conference on Learning Representations}. Rio de Janeiro, Brazil: OpenReview.net; 2026.

\bibitem{deepst_2022}
Xu C, Jin X, Wei S \textit{et al}. DeepST: identifying spatial domains in spatial transcriptomics by deep learning. \textit{Nucleic Acids Res} 2022;\textbf{50}:e131.

\bibitem{ferreira2025selfsupervised}
Ferreira DL, Lau C, Salaymang Z \textit{et al}. Self-supervised learning for label-free segmentation in cardiac ultrasound. \textit{Nat Commun} 2025;\textbf{16}:4070.

\bibitem{cui2024scgpt}
Cui H, Wang C, Maan H \textit{et al}. scGPT: toward building a foundation model for single-cell multi-omics using generative AI. \textit{Nat Methods} 2024;\textbf{21}:1470--80.

\bibitem{crossmodal_cardiac_ae_2023}
Radhakrishnan A, Friedman SF, Khurshid S \textit{et al}. Cross-modal autoencoder framework learns holistic representations of cardiovascular state. \textit{Nat Commun} 2023;\textbf{14}:2436.

\bibitem{radford2021_clip}
Radford A, Kim JW, Hallacy C \textit{et al.} Learning transferable visual models from natural language supervision. In: \textit{Proceedings of the} \textit{38th International Conference on Machine Learning}. Virtual conference: Proceedings of Machine Learning Research; 2021. 139:8748--63.

\bibitem{zhang2022_convirt}
Zhang Y, Jiang H, Miura Y \textit{et al.} Contrastive learning of medical visual representations from paired images and text. In: Proceedings \textit{of the 7th Machine Learning for Healthcare Conference}. Durham (NC), USA: \textit{Proceedings} of Machine Learning Research; 2022. 182:2--25.

\bibitem{foundation_radiology_2025}
Akinci D'Antonoli T, Bluethgen C, Cuocolo R \textit{et al.} Foundation models for radiology: fundamentals, applications, opportunities, challenges, risks, and prospects. \textit{Diagn Interv Radiol} 2026;\textbf{32}:259--72.

\bibitem{sun2024_medical_mmfm}
Sun K, Xue S, Sun F \textit{et al.} Medical multimodal foundation models in clinical diagnosis and treatment: applications, challenges, and future directions. \textit{Artif Intell Med} 2025;\textbf{170}:103265.

\bibitem{strotzer2024_gpt4v_radiology}
Strotzer QD, Nieberle F, Kupke LS \textit{et al}. Toward foundation models in radiology? Quantitative assessment of GPT-4V's multimodal and multianatomic region capabilities. \textit{Radiology} 2024;\textbf{313}: e240955.

\bibitem{abbasi2024deep}
Abbasi S, Lan H, Choupan J \textit{et al}. Deep learning for the harmonization of structural MRI scans: a survey. \textit{Biomed Eng Online} 2024;\textbf{23}:90.

\bibitem{johnson2007_combat}
Johnson WE, Li C, Rabinovic A. Adjusting batch effects in microarray expression data using empirical bayes methods. \textit{Biostatistics} 2007;\textbf{8}:118--27.

\bibitem{korsunsky2019_harmony}
Korsunsky I, Millard N, Fan J \textit{et al}. Fast, sensitive and accurate integration of single-cell data with harmony. \textit{Nat Methods} 2019;\textbf{16}:1289--96.

\bibitem{hassani2020myocardial}
Hassani C, Saremi F, Varghese BA \textit{et al}. Myocardial radiomics in cardiac MRI. \textit{Am J Roentgenol} 2020;\textbf{214}:536--45.

\bibitem{bhattacharya2022multi}
Bhattacharya A, Sadasivuni S, Chao C-J \textit{et al}. Multi-modal fusion model for predicting adverse cardiovascular outcome post percutaneous coronary intervention. \textit{Physiol Meas} 2022;\textbf{43}:124004.

\bibitem{baltrusaitis2019_multimodal}
Baltrušaitis T, Ahuja C, Morency L-P. Multimodal machine learning: a survey and taxonomy. \textit{IEEE Trans Pattern Anal Mach Intell} 2019;\textbf{41}:423--43.

\bibitem{andrew2013_dcca}
Andrew G, Arora R, Bilmes J \textit{et al.} Deep canonical correlation analysis. In: \textit{Proceedings of the 30th International Conference on Machine} Learning. Atlanta (GA), USA: Proceedings of Machine \textit{Learning} Research; 2013. 28:1247--55.

\bibitem{wang2015_dccae}
Wang W, Arora R, Livescu K \textit{et al.} On deep multi-view representation learning. In: \textit{Proceedings of the 32nd International Conference on} Machine Learning. Lille, France: Proceedings of \textit{Machine Learning} Research; 2015. 37:1083--92.

\bibitem{wu2018_multimodal_vae}
Wu M, Goodman N. Multimodal generative models for scalable weakly-supervised learning. In: \textit{Advances in Neural Information} \textit{Processing Systems (NeurIPS)} 2018;\textbf{31}:5580--90.

\bibitem{joshi2022generalized}
Joshi A, Gupta N, Shah J \textit{et al.} Generalized product-of-experts for learning multimodal representations in noisy environments. In: \textit{Proceedings of the 2022 International Conference on Multimodal} \textit{Interaction}. Bengaluru, India: Association for Computing Machinery; 2022. p. 83--93.

\bibitem{hemker2024healnet}
Hemker K, Simidjievski N, Jamnik M. HEALNet: multimodal fusion for heterogeneous biomedical data. \textit{Adv Neural Inf Process Syst} 2024;\textbf{37}:64479--98.

\bibitem{tonekaboni2025representation}
Tonekaboni S, Friedman SF, Zhang X \textit{et al}. A representation fusion framework for decoupling diagnostic information in multimodal learning. \textit{NPJ Digit Med} 2025;\textbf{8}:765.

\bibitem{zheng2024graph}
Zheng Y, Conrad RD, Green EJ \textit{et al}. Graph attention-based fusion of pathology images and gene expression for prediction of cancer survival. \textit{IEEE Trans Med Imaging} 2024;\textbf{43}:3085--97.

\bibitem{li2025graph}
Li S, Hua H, Chen S. Graph neural networks for single-cell omics data: a review of approaches and applications. \textit{Brief Bioinform} 2025;\textbf{26}:bbaf109.

\bibitem{parisot2018_gnn_brain}
Parisot S, Ktena SI, Ferrante E \textit{et al.} Disease prediction using graph convolutional networks: application to autism spectrum disorder and Alzheimer's disease. \textit{Med Image Anal} 2018;\textbf{48}:117--30.

\bibitem{chen2022pan}
Chen RJ, Lu MY, Williamson DFK \textit{et al}. Pan-cancer integrative histology-genomic analysis via multimodal deep learning. \textit{Cancer} \textit{Cell} 2022;\textbf{40}:865--78.

\bibitem{howard2023multimodal}
Howard FM, Kather JN, Pearson AT. Multimodal deep learning: an improvement in prognostication or a reflection of batch effect? \textit{Cancer Cell} 2023;\textbf{41}:5--6.

\bibitem{vickers2006_decision_curve}
Vickers AJ, Elkin EB. Decision curve analysis: a novel method for evaluating prediction models. \textit{Med Decis Making} 2006;\textbf{26}:565--74.

\bibitem{tripod_ai_2024}
Collins GS, Dhiman P, Andaur CL \textit{et al}. TRIPOD+AI: updated guidance for reporting clinical prediction models that use machine learning. \textit{BMJ} 2024;\textbf{385}:e078378.

\bibitem{moons2025probast}
Moons KGM, Damen JAA, Kaul T \textit{et al.} PROBAST+AI: an updated quality, risk of bias, and applicability assessment tool for prediction models using regression or artificial intelligence methods. \textit{BMJ} 2025;\textbf{388}:e082505.

\bibitem{argelaguet2020_mofa_plus}
Argelaguet R, Arnol D, Bredikhin D \textit{et al}. MOFA+: a statistical framework for comprehensive integration of multi-modal single-cell data. \textit{Genome Biol} 2020;\textbf{21}:111.

\bibitem{palla2022_squidpy}
Palla G, Spitzer H, Klein M \textit{et al}. Squidpy: a scalable framework for spatial omics analysis. \textit{Nat Methods} 2022;\textbf{19}:171--8.

\bibitem{dries2021_giotto}
Dries R, Zhu Q, Dong R \textit{et al}. Giotto: a toolbox for integrative analysis and visualization of spatial expression data. \textit{Genome Biol} 2021;\textbf{22}:78.

\bibitem{monai2022}
The MONAI Consortium. MONAI: Medical Open Network for AI. \textit{arXiv preprint arXiv:2211.02701}. Ithaca (NY): Cornell University; 2022.

\bibitem{perezgarcia2021_torchio}
Pérez-García F, Sparks R, Ourselin S. TorchIO: a Python library for efficient loading, preprocessing, augmentation and patch-based sampling of medical images in deep learning. \textit{Comput Methods Prog} \textit{Biomed} 2021;\textbf{208}:106236.

\bibitem{he2024radiogenomics}
He W, Huang W, Zhang L \textit{et al}. Radiogenomics: bridging the gap between imaging and genomics for precision oncology. \textit{MedComm} 2024;\textbf{5}:e722.

\bibitem{guo2025images}
Guo Y, Li T, Gong B \textit{et al}. From images to genes: radiogenomics based on artificial intelligence to achieve non-invasive precision medicine in cancer patients. \textit{Adv Sci} 2025;\textbf{12}:2408069.

\bibitem{lin2025machine}
Lin M, Guo J, Gu Z \textit{et al}. Machine learning and multi-omics integration: advancing cardiovascular translational research and clinical practice. \textit{J Transl Med} 2025;\textbf{23}:388.

\bibitem{infante2021radiogenomics}
Infante T, Cavaliere C, Punzo B \textit{et al}. Radiogenomics and artificial intelligence approaches applied to cardiac computed tomography angiography and cardiac magnetic resonance for precision medicine in coronary heart disease: a systematic review. \textit{Circ} \textit{Cardiovasc Imaging} 2021;\textbf{14}:1133--46.

\bibitem{ho2018genotype}
Ho CY, Day SM, Ashley EA \textit{et al}. Genotype and lifetime burden of disease in hypertrophic cardiomyopathy: insights from the sarcomeric human cardiomyopathy registry (SHaRe). \textit{Circulation} 2018;\textbf{138}:1387--98.

\bibitem{wehrens2022single}
Wehrens M, de Leeuw AE, Wright-Clark M \textit{et al.} Single-cell transcriptomics provides insights into hypertrophic cardiomyopathy. \textit{Cell Rep} 2022;\textbf{39}:110809.

\bibitem{ahlberg2024_cmr_gwas}
Ahlberg G, Andreasen L, Ghouse J \textit{et al}. Genome-wide association study identifies 18 novel loci associated with left atrial volume and function. \textit{Eur Heart J} 2021;\textbf{42}:4523--34.

\bibitem{luo2026ai}
Luo Y, Zhang N, Yang J \textit{et al.} AI-based multiomics profiling reveals complementary omics contributions to personalized prediction of cardiovascular disease. \textit{Nat Commun} 2026;\textbf{17}:2269.

\bibitem{khan2025comprehensive}
Khan M, Arslanturk S, Draghici S. A comprehensive review of spatial transcriptomics data alignment and integration. \textit{Nucleic} \textit{Acids Res} 2025;\textbf{53}:gkaf536.

\bibitem{ekvall2024spatial}
Ekvall M, Bergenstråhle L, Andersson A \textit{et al}. Spatial landmark detection and tissue registration with deep learning. \textit{Nat Methods} 2024;\textbf{21}:673--9.

\bibitem{chelebian2025combining}
Chelebian E, Avenel C, Wählby C. Combining spatial transcriptomics with tissue morphology. \textit{Nat Commun} 2025;\textbf{16}:4452.

\bibitem{fu2025spatial}
Fu X, Cao Y, Bian B \textit{et al}. Spatial gene expression at single-cell resolution from histology using deep learning with GHIST. \textit{Nat} \textit{Methods} 2025;\textbf{22}:1900--10.

\bibitem{raghunath2020prediction}
Raghunath S, Ulloa AE, Cerna LJ \textit{et al}. Prediction of mortality from 12-lead electrocardiogram voltage data using a deep neural network. \textit{Nat Med} 2020;\textbf{26}:886--91.

\bibitem{attia2019artificial}
Attia ZI, Noseworthy PA, Lopez-Jimenez F \textit{et al}. An artificial intelligence-enabled ECG algorithm for the identification of patients with atrial fibrillation during sinus rhythm: a retrospective analysis of outcome prediction. \textit{Lancet} 2019; \textbf{394}:861--7.

\bibitem{sau2024artificial}
Sau A, Pastika L, Sieliwonczyk E \textit{et al}. Artificial intelligence-enabled electrocardiogram for mortality and cardiovascular risk estimation: a model development and validation study. \textit{Lancet Digit} \textit{Health} 2024;\textbf{6}:e791--802.

\bibitem{vukadinovic2026echoprime}
Vukadinovic M, Chiu I-M, Tang X \textit{et al}. Comprehensive echocardiogram evaluation with view primed vision language AI. \textit{Nature} 2026;\textbf{650}:970--7.

\bibitem{forrest2023machine}
Forrest IS, Petrazzini BO, Duffy Á \textit{et al}. Machine learning-based marker for coronary artery disease: derivation and validation in two longitudinal cohorts. \textit{Lancet} 2023;\textbf{401}:215--25.

\bibitem{lai2025multimodal}
Lai C, Yin M, Kholmovski EG \textit{et al}. Multimodal AI to forecast arrhythmic death in hypertrophic cardiomyopathy. \textit{Nat Cardiovasc} \textit{Res} 2025;\textbf{4}:891--903.

\bibitem{sushil2025_miclaim_gen}
Miao BY, Chen IY, Williams CYK \textit{et al}. The MI-CLAIM-GEN checklist for generative artificial intelligence in health. \textit{Nat Med} 2025;\textbf{31}:1394--8.

\bibitem{acosta2022multimodal}
Acosta JN, Falcone GJ, Rajpurkar P \textit{et al}. Multimodal biomedical AI. \textit{Nat Med} 2022;\textbf{28}:1773--84.

\bibitem{quer2024_llm_cardiovascular_medicine}
Quer G, Topol EJ. The potential for large language models to transform cardiovascular medicine. \textit{Lancet Digit Health} 2024;\textbf{6}: e767--71.

\bibitem{sarraju2023_llm_cardiology}
Sarraju A, Ouyang D, Itchhaporia D. The opportunities and challenges of large language models in cardiology. \textit{JACC: Advances} 2023;\textbf{2}:100438.

\bibitem{eu_ai_act_2024}
European Parliament and Council of the European Union. Regulation (EU) 2024/1689 of 13 June 2024 laying down harmonised rules on artificial intelligence (Artificial Intelligence Act). \textit{Official Journal of the European Union 2024;L 2024/1689}. Luxembourg: Publications Office of the European Union; 2024.

\bibitem{norouzi2025dft_anpd}
Norouzi R, Norouzi R, Abbasi K \textit{et al}. DFT\_ANPD: a dual-feature two-sided attention network for anticancer natural products detection. \textit{Comput Biol Med} 2025;\textbf{194}:110442.

\bibitem{abbasi2020_partwhole_fcn}
Abbasi K, Razzaghi P. Incorporating part-whole hierarchies into fully convolutional network for scene parsing. \textit{Expert Syst Appl} 2020;\textbf{160}:113662.

\bibitem{dmytrenko2025_comp_drug_design_review}
Abbasi K, Razzaghi P, Gharizadeh A \textit{et al}. Computational drug design in the artificial intelligence era: a systematic review of molecular representations, generative architectures, and performance assessment. \textit{Pharmacol Rev} 2026;\textbf{78}:100095.

\bibitem{corralacero2020_precision_cardiology}
Corral-Acero J, Margara F, Marciniak M \textit{et al}. The 'digital twin' to enable the vision of precision cardiology. \textit{Eur Heart J} 2020;\textbf{41}:4556--64.

\bibitem{coorey2022_health_digital_twin}
Coorey GM, Figtree GA, Fletcher DF \textit{et al}. The health digital twin to tackle cardiovascular disease---a review of an emerging interdisciplinary field. \textit{NPJ Digit Med} 2022;\textbf{5}:126.

\bibitem{prakosa2018personalized}
Prakosa A, Arevalo HJ, Deng D \textit{et al}. Personalized virtual-heart technology for guiding the ablation of infarct-related ventricular tachycardia. \textit{Nat Biomed Eng} 2018;\textbf{2}:732--40.

\bibitem{sel2024_building_digital_twins}
Sel K, Osman D, Zare F \textit{et al}. Building digital twins for cardiovascular health: from principles to clinical impact. \textit{J Am Heart Assoc} 2024;\textbf{13}:e031981.

\bibitem{akbarialiabad2025_insilico_trials}
Akbarialiabad H, Pasdar A, Murrell DF \textit{et al}. Enhancing randomized clinical trials with digital twins. \textit{NPJ Syst Biol Appl} 2025;\textbf{11}:110.

\bibitem{arevalo2016arrhythmia}
Arevalo HJ, Vadakkumpadan F, Guallar E \textit{et al}. Arrhythmia risk stratification of patients after myocardial infarction using personalized heart models. \textit{Nat Commun} 2016;\textbf{7}:11437.
\end{thebibliography}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/tables/table-1.tex <==
\begin{table*}[!tp]
\centering
\sffamily\fontsize{7.5bp}{9.45bp}\selectfont
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1}
\caption{Public multimodal cardiology datasets relevant to imaging-anchored multiomics, including resources that directly pair cardiovascular imaging with molecular data and adjacent multimodal cardiovascular resources useful for encoder pretraining and transfer learning.}
\label{tab:multimodal_cardiology_datasets}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{\dimexpr 0.15645\textwidth - 2.500pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.15090\textwidth - 2.500pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.15090\textwidth - 2.500pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.27576\textwidth - 2.500pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.17809\textwidth - 2.500pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.08790\textwidth - 2.500pt\relax}@{}}
\toprule
\textbf{Dataset/study} & \textbf{Type} & \textbf{Cardiovascular focus} & \textbf{Modalities included} & \textbf{Approximate scale and access} & \textbf{Link} \\
\midrule
UK Biobank imaging extension \cite{petersen2013imaging} &
Population imaging cohort &
Cardiac structure, function, and risk in mid-life adults &
CMR, vascular ultrasound and other MRI sequences linked to genome-wide genotyping, exome sequencing, plasma proteomics, metabolomics, EHR, and questionnaires &
$\sim$100,000 participants with CMR and >500,000 with genomics; application-based access &
\href{https://www.ukbiobank.ac.uk/}{UK Biobank} \\[1.5pt]
Multi-Ethnic Study of Atherosclerosis (MESA) \cite{bild2002_mesa} &
Population cohort with multimodal imaging &
Subclinical atherosclerosis and incident CVD in a diverse community sample &
CMR, coronary artery calcium CT, carotid ultrasound, and other imaging linked to genotype, labs, and risk-factor profiling &
$\sim$6,800 participants; controlled access via NHLBI repositories &
\href{https://biolincc.nhlbi.nih.gov/studies/mesa/}{BioLINCC} \\[1.5pt]
Hypertrophic Cardiomyopathy Registry (HCMR) \cite{kramer2015_hcmr} &
Disease registry and biobank &
Risk stratification in hypertrophic cardiomyopathy &
CMR, echocardiography and electrocardiography (ECG) combined with targeted gene sequencing and circulating biomarkers &
$\sim$2,700 patients; collaborative access via data-use agreements &
\href{https://www.hcmregistry.org/}{HCMR} \\[1.5pt]
MIMIC-IV and related PhysioNet modules \cite{gow2023_mimic_iv_ecg} &
Critical-care waveform and EHR resource &
Acute CVD and haemodynamic instability in ICU/ED settings &
Twelve-lead ECG waveforms linked to high-resolution EHR; additional echo and note modules for subsets &
$\sim$800,000 ECGs in $\sim$160,000 subjects; credentialed access via PhysioNet &
\href{https://physionet.org/content/mimiciv/3.1/}{PhysioNet} \\[1.5pt]
EchoNet family (EchoNet-Dynamic, EchoNet-LVH) \cite{ouyang2020_echonet_dynamic,duffy2022high} &
Curated echocardiography video datasets &
LV systolic function, wall motion, and hypertrophy phenotypes &
Apical four-chamber echo videos with contour tracings, volumetric measurements, and labels (EF, LVH) &
On the order of $10^{4}$ videos; de-identified datasets downloadable for research &
\href{https://echonet.github.io/dynamic/}{EchoNet} \\[1.5pt]
Cardiac Atlas Project CMR cohorts \cite{fonseca2011_cardiac_atlas} &
Aggregated CMR repositories &
Cardiac structure and function in health and early disease &
3D cine CMR studies with segmentations, finite-element meshes and clinical covariates in selected cohorts &
Thousands of CMR exams; access under data-use agreements &
\href{https://www.cardiacatlas.org/}{Cardiac Atlas} \\[1.5pt]
Spatial multi-omic map of human myocardial infarction \cite{kuppe2022_spatial_mi} &
Human tissue atlas with single-cell and spatial multiomics &
Early and late remodelling after acute myocardial infarction &
snRNA-seq, snATAC-seq, Visium spatial transcriptomics, and matched histology across infarct core, border zone, and remote myocardium &
31 samples from 23 patients; processed data via public portals and archives &
\href{https://data.humancellatlas.org/}{HCA portal} \\[1.5pt]
Coronary plaque spatial transcriptomics studies \cite{campos2025_spatial_plaque,sun2023spatial,gastanadui2024_coronary_spatial_plaque} &
Plaque-level spatial-omics studies &
Plaque stability, inflammatory niches, and high-risk morphologies &
Spatial transcriptomics of human coronary arteries with histology and plaque morphology; some cohorts include CT or invasive imaging &
Dozens of plaques; expression matrices; and metadata commonly deposited to GEO/ENA (see articles) &
\href{https://www.ncbi.nlm.nih.gov/geo/}{GEO} \\[1.5pt]
\bottomrule
\end{tabular}
\end{table*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/tables/table-2.tex <==
\begin{table*}[!tp]
\centering
\sffamily\fontsize{7.5bp}{9.45bp}\selectfont
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1}
\caption{Representative cardiovascular imaging biomarkers that often serve as anchors in imaging-anchored multiomics, with typical computational extraction strategies and plausible molecular correlates.}
\label{tab:imaging_biomarkers}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{\dimexpr 0.22271\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.23880\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.23880\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.29969\textwidth - 2.250pt\relax}@{}}
\toprule
\textbf{Biomarker (modality)} & \textbf{Clinical interpretation} & \textbf{Typical computational extraction} & \textbf{Plausible or reported molecular correlates} \\
\midrule
LGE extent and pattern (CMR) \cite{kuruvilla2014_lge_meta} &
Focal myocardial scar/fibrosis; arrhythmic and HF risk &
Segmentation of LGE-positive regions; regional burden by AHA segments; texture/radiomics &
Fibroblast activation, collagen deposition (ECM programmes), immune infiltration in border zones; stress and remodelling programmes in cardiomyocytes \\[1.5pt]
Global longitudinal strain (echo) \cite{kalam2014_gls_meta} &
Subclinical systolic dysfunction; prognostic across many CVD states &
Speckle-tracking strain curves; regional strain maps; video encoders for deformation fields &
Energetic stress, sarcomeric dysfunction, inflammatory signalling; chamber-specific cardiomyocyte stress responses \\[1.5pt]
Low-attenuation noncalcified plaque (coronary CTA) \cite{williams2020_scotheart_lap} &
Lipid-rich plaque; higher MI risk &
Plaque segmentation and attenuation profiling; radiomics; phenotype classifiers &
Macrophage-driven inflammation, necrotic core formation, matrix remodelling; immune niches at plaque shoulders \\[1.5pt]
Napkin-ring sign/high-risk plaque morphology (CTA) \cite{otsuka2013_napkin_ring} &
High-risk plaque architecture; potential plaque vulnerability &
CNN/ViT-based plaque morphology classification; handcrafted geometry features &
Protease and cytokine signalling, macrophage activation, smooth muscle cell phenotypic switching; local hypoxia \\[1.5pt]
Perivascular fat attenuation index (FAI) (CTA) \cite{oikonomou2018_pv_fai_risk} &
Non-invasive readout of coronary inflammation &
Perivascular fat segmentation; attenuation gradients; radiotranscriptomic mapping &
Inflammatory adipose and vascular wall transcripts; cytokine signalling and fibrosis-related programmes \\[1.5pt]
\bottomrule
\end{tabular}
\end{table*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/tables/table-3.tex <==
\begin{table*}[!tp]
\centering
\sffamily\fontsize{7.5bp}{9.45bp}\selectfont
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1}
\caption{Practical comparison of traditional unimodal/low-dimensional modelling versus multimodal fusion strategies for imaging-anchored multi-omics.}
\label{tab:fusion_comparison}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{\dimexpr 0.23344\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.28782\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.26044\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.21831\textwidth - 2.250pt\relax}@{}}
\toprule
\textbf{Approach} & \textbf{Strengths} & \textbf{Common failure modes} & \textbf{When it is a good default} \\
\midrule
Classical regression/survival models with hand-crafted radiomics summaries &
High interpretability; strong calibration; stable in small samples &
Limited ability to capture spatial heterogeneity and cross-modal interactions; features may miss subtle biology &
Early translational work; limited paired data; when interpretability and calibration dominate \\[1.5pt]
Early fusion (feature concatenation) &
Simple; uses standard ML toolkits; often competitive baselines &
Sensitive to missing modalities; scaling/normalization issues; collinearity, and overfitting with high-dimensional omics &
Moderate sample sizes with mostly complete modalities; when a strong baseline is needed quickly \\[1.5pt]
Intermediate fusion (joint latent space: DCCA, multimodal VAE, and HEALNet) &
Captures non-linear cross-modal interactions; supports ``virtual omics'' and mechanistic exploration; handles missing modalities via product-of-experts &
Latent space collapse; modality imbalance; requires careful regularization and validation &
When paired subsets exist but are not large; when cross-modal generation/interpretation is desired \\[1.5pt]
Late fusion (ensembles/stacking) &
Robust to missing modalities; reuses validated unimodal models; simplifies regulatory adoption &
Cannot learn feature-level synergy; may underperform when cross-modal interactions are important; forfeits opportunity to learn from costly paired data &
When missingness is high; when unimodal models are already mature and well-validated; as deployment fallback \\[1.5pt]
Graph/contrastive and transformer-based fusion &
Naturally incorporates spatial and biological priors; can scale with pretraining; captures neighbourhood relationships lost by flat vectors &
Data-hungry; computationally expensive; prone to spurious shortcuts without strong evaluation &
When large weakly labelled data exist for pretraining, or strong spatial/biological graphs are available \\[1.5pt]
\bottomrule
\end{tabular}
\end{table*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/tables/table-4.tex <==
\begin{table*}[!tp]
\centering
\sffamily\fontsize{7.5bp}{9.45bp}\selectfont
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1}
\caption{Evaluation metrics and validation designs commonly used (or recommended) in imaging-anchored multiomics.}
\label{tab:evaluation_metrics}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{\dimexpr 0.17733\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.23171\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.28591\textwidth - 2.250pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.30506\textwidth - 2.250pt\relax}@{}}
\toprule
\textbf{Task} & \textbf{Example outputs} & \textbf{Useful metrics} & \textbf{Validation emphasis} \\
\midrule
Clinical prediction/risk modelling &
Binary outcome, time-to-event risk, treatment response &
AUC/time-dependent AUC, C-index, Brier score; calibration slope/curve; decision-curve net benefit \cite{vickers2006_decision_curve} &
External validation; leave-one-site-out; calibration and subgroup performance; reporting per TRIPOD+AI/PROBAST+AI \cite{moons2025probast} \\[1.5pt]
Radiogenomic association &
Imaging feature $\leftrightarrow$ gene/pathway score &
Effect sizes, false discovery rate control; pathway enrichment; replication rate &
Confounder adjustment; permutation tests; replication in independent cohorts \\[1.5pt]
Cross-modal alignment/retrieval &
Paired embeddings; matched region--spot correspondences &
Cross-modal retrieval (Recall@K), embedding correlation/CCA correlation, alignment error &
Robustness to missing modalities; negative controls (shuffled pairing); sensitivity to batch \\[1.5pt]
Spatial domain discovery &
Spot clusters/spatial domains &
Adjusted Rand index (if labels exist), silhouette score; spatial autocorrelation statistics &
Stability under downsampling; cross-section reproducibility; biological plausibility via marker genes \\[1.5pt]
Virtual transcriptomics &
Predicted gene/module expression maps &
Pearson/Spearman correlation, $R^2$, RMSE; spatial pattern similarity &
Hold-out donors/centres; robustness across staining/scanner protocols; uncertainty estimates \\[1.5pt]
\bottomrule
\end{tabular}
\end{table*}


==> BIB_Review_Bioinformatics_MinhLe_UPDATED/tables/table-5.tex <==
\begin{table*}[!tp]
\centering
\sffamily\fontsize{7.5bp}{9.45bp}\selectfont
\setlength{\tabcolsep}{1.5pt}
\renewcommand{\arraystretch}{1}
\caption{Representative frameworks and studies integrating cardiovascular imaging with molecular or other high-dimensional omic data, including general-purpose frameworks that have been applied or are directly applicable to imaging-anchored multiomics and cardiovascular studies that exemplify concrete imaging--omics applications in cardiology.}
\label{tab:imaging_omics_frameworks}
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{\dimexpr 0.15760\textwidth - 2.400pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.20069\textwidth - 2.400pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.23899\textwidth - 2.400pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.21160\textwidth - 2.400pt\relax}>{\raggedright\arraybackslash}p{\dimexpr 0.19111\textwidth - 2.400pt\relax}@{}}
\toprule
\textbf{Framework/study} & \textbf{Modalities integrated} & \textbf{Integration strategy} & \textbf{Cardiovascular relevance - example use} & \textbf{Key contribution} \\
\midrule
\multicolumn{5}{@{}l}{\textit{General-purpose multimodal frameworks applicable to imaging--omics integration}} \\[2pt]
MOFA+, scVI/totalVI, and scvi-tools \cite{lopez2018_scvi,gayoso2022_scvi_tools,argelaguet2020_mofa_plus} &
Bulk and single-cell transcriptomics, epigenomics, proteomics; imaging-derived features can be included as an additional view &
Probabilistic factor models (MOFA+) and hierarchical VAEs (scVI) that learn joint low-dimensional representations while explicitly modelling batch effects and missing data &
Provide molecular latent spaces---shared factors or scVI latent variables---that can be aligned with cardiac imaging embeddings for radiogenomic and spatial integration &
Established ecosystem with documented APIs; standard entry point for cardiovascular multiomics before fusion with imaging \\[1.5pt]
Multimodal VAEs \cite{wu2018_multimodal_vae,joshi2022generalized} &
Heterogeneous combinations of imaging, omics, and clinical data &
Product-of-experts or mixture-of-experts aggregation of modality-specific encoder posteriors into a shared latent space; joint posterior remains well-defined when modalities are missing &
Prototype framework for learning shared imaging--omics latent spaces; supports ``virtual omics'' generation from imaging inputs alone &
Handle missing modalities by design; probabilistic formulation enables uncertainty quantification and cross-modal simulation \\[1.5pt]
PORPOISE \cite{chen2022pan} &
Whole-slide H\&E histopathology and multi-omic profiles (RNA-seq, CNV, mutations) across 14 TCGA cancer types &
Attention-based multiple instance learning (MIL) for whole-slide images (WSIs) fused with a self-normalizing network for omics via Kronecker-product gated fusion; weakly supervised with survival labels &
Architecturally transferable to cardiac histology--omics; interpretable morpho-molecular prognostic markers at pan-cancer scale &
First large-scale interpretable histology--genomic fusion; open-source code and interactive atlas; highlighted batch-effect risks in site-unaware splits \cite{howard2023multimodal} \\[1.5pt]
HEALNet \cite{hemker2024healnet} &
Whole-slide histopathology and multi-omic data (four TCGA cancer datasets) &
Iterative cross-attention between a shared latent bottleneck and modality-specific token streams; processes raw inputs rather than precomputed embeddings &
Directly applicable to cardiac tissue sections with matched omics; handles missing modalities at both training and inference &
State-of-the-art survival prediction among end-to-end fusion models; open-source; modular design facilitates addition of imaging modalities \\[1.5pt]
\addlinespace[3pt]
\multicolumn{5}{@{}l}{\textit{Cardiovascular imaging--omics studies}} \\[2pt]
Cross-modal autoencoder for cardiovascular state \cite{crossmodal_cardiac_ae_2023} &
Twelve-lead ECG, CMR cine images and clinical traits from the UK Biobank &
Cross-modal autoencoder reconstructing each modality from a shared latent vector; supports imputation of missing modalities and genotype association in latent space &
Phenotype prediction, unsupervised GWAS, and CMR imputation from ECG at population scale (n > 40,000) &
Scalable cross-modal representation learning linking low-cost ECG signals to rich CMR phenotypes and genetic architecture \\[1.5pt]
MODES \cite{tonekaboni2025representation} &
Twelve-lead ECG and CMR from the UK Biobank &
Representation fusion framework decoupling shared and modality-specific latent components via orthogonality constraints &
Inference of missing MRI phenotypes from ECG alone; shared latent captures interpretable cardiac structure--function relationships &
Explicit shared/private decomposition improves cross-modal prediction and clinical interpretability in cardiovascular data \\[1.5pt]
Radiotranscriptomic perivascular fat signature \cite{oikonomou2018_pv_fai_risk,oikonomou2019novel} &
Coronary CTA radiomics of perivascular fat and microarray gene-expression from perivascular adipose biopsies &
Machine-learning mapping of CT radiomic features onto tissue gene-expression modules to derive a radiotranscriptomic risk score &
Prediction of cardiac mortality and MI beyond standard CT and clinical risk scores in coronary CTA cohorts &
Proof-of-concept that CT radiomics can serve as a non-invasive surrogate for local vascular inflammatory and fibrotic gene-expression states \\[1.5pt]
Spatial multi-omic map of human myocardial infarction \cite{kuppe2022_spatial_mi} &
snRNA-seq, snATAC-seq, Visium spatial transcriptomics, and histology of infarcted and control myocardium &
Joint embedding of single-cell and spatial omics to annotate infarct core, border and remote zones with dominant cell states and regulatory programmes &
Mechanistic dissection of human MI remodelling across regions and time points; tissue blocks sampled from imaging-defined zones &
Tissue-scale molecular atlas co-registrable with imaging markers of infarct size, scar distribution and remodelling \\[1.5pt]
Coronary plaque spatial transcriptomics linked to imaging \cite{campos2025_spatial_plaque,sun2023spatial,gastanadui2024_coronary_spatial_plaque} &
Spatial transcriptomics of human coronary plaques with matched histology; invasive or CT imaging in selected cohorts &
Spatial co-localization of gene-expression modules and immune niches with plaque morphology and CT features such as low-attenuation plaque or thin-cap fibroatheroma &
Characterization of high-risk plaque phenotypes and local immune microenvironments in coronary artery disease &
Template for connecting coronary imaging markers of vulnerability with spatially resolved arterial wall gene-expression and immune niches \\[1.5pt]
\bottomrule
\end{tabular}
\end{table*}

